Regression Type Models for Extremal Dependence

We propose a vector generalized additive modeling framework for taking into account the effect of covariates on angular density functions in a multivariate extreme value context. The proposed methods are tailored for settings where the dependence between extreme values may change according to covariates. We devise a maximum penalized log-likelihood estimator, discuss details of the estimation procedure, and derive its consistency and asymptotic normality. The simulation study suggests that the proposed methods perform well in a wealth of simulation scenarios by accurately recovering the true covariate-adjusted angular density. Our empirical analysis reveals relevant dynamics of the dependence between extreme air temperatures in two alpine resorts during the winter season. Supplementary materials for this article are available online.

==> Regression_Type_Models_for_Extremal_Dependence 2/Latex/colors.tex <==
\usepackage{color}

\def\red#1{{\color{red} #1}}%
\def\blue#1{{\color{blue} #1}}%
\def\green#1{{\color{green} #1}}

% \newcommand{\Cexpr}[1]{\blue{\Sexpr{#1}}}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> Regression_Type_Models_for_Extremal_Dependence 2/Latex/environments.tex <==
% Theorem-like structures
\newtheorem{theorem}{Theorem}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}
\newtheorem{proposition}{Proposition}
\newtheorem{conjecture}{Conjecture}
\newtheorem{corollary}[theorem]{Corollary} 
\newtheorem{lemma}{Lemma}
\newtheorem{remark}{Remark}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> Regression_Type_Models_for_Extremal_Dependence 2/Latex/header.tex <==
%%% MATH, FIGURES AND DISPLAY PACKAGES
%\usepackage[latin1]{inputenc}
\usepackage{url}
\usepackage{amsmath,amsfonts,amssymb,amscd,mathtools,bm,bbm}
\usepackage{multirow,tabularx,subfig,graphicx}
\usepackage{tikz}
\usetikzlibrary{calc,trees,positioning,arrows,chains,shapes.geometric, decorations.pathreplacing,decorations.pathmorphing,shapes, matrix,shapes.symbols}
\tikzset{ >=stealth', punktchain/.style={ rectangle, rounded corners, draw=black, very thick, text width=10em, minimum height=3em, text centered, on chain}}

%%% SPECIAL COMMANDS AND DEFINITIONS
\newcommand{\greekvec}[1]{\mbox{\boldmath$#1$}}
\newcommand{\IR}{\mathbbm{R}}
\newcommand{\vtheta}{\greekvec{\theta}}
\newcommand{\vgamma}{\greekvec{\gamma}}
\newcommand{\vepsilon}{\greekvec{\varepsilon}}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\def\toD{\buildrel d\over\rightarrow}
\def\toP{\buildrel p\over\rightarrow}
\def\eqD{\buildrel d\over =}
\newcommand{\omegaV}{\mbox{\boldmath \(\omega\)}}
\newcommand{\alphaV}{\mbox{\boldmath \(\alpha\)}}
\newcommand{\thetaV}{\mbox{\boldmath \(\theta\)}}
\newcommand{\PsiV}{\mbox{\boldmath \(\Psi\)}}
\newcommand{\psiV}{\mbox{\boldmath \(\psi\)}}
\newcommand{\gammaV}{\mbox{\boldmath \(\gamma\)}}


==> Regression_Type_Models_for_Extremal_Dependence 2/Latex/short_bib.tex <==
% To shorten the reference list use:
 \let\oldthebibliography=\thebibliography
 \let\oldendthebibliography=\endthebibliography
 \renewenvironment{thebibliography}[1]{%
   \footnotesize
   \oldthebibliography{#1}%
   \setlength{\parskip}{0mm}%
   \setlength{\itemsep}{0mm}%
 }{\oldendthebibliography}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> Regression_Type_Models_for_Extremal_Dependence 2/Latex/tools.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                      Math                                    %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Calculus
\newcommand{\e}{\mathrm{e}}
\newcommand{\dif}{\ensuremath{\mathrm{d}}}
\newcommand{\nto}{\ensuremath{\underset{n \to \infty}{\rightarrow}}}
% \def\tsum{\mathop{\textstyle \sum }}
% \def\tprod{\mathop{\textstyle \prod }}
% \def\tint{\mathop{\textstyle \int}}
% Linear Algebra
\newcommand{\T}{\ensuremath{\mathrm{\scriptscriptstyle T}}}
% Bold Greek Uppercase
\usepackage{bm}
\newcommand{\Gammab}{\ensuremath{\bm\Gamma}}
\newcommand{\Deltab}{\ensuremath{\bm\Delta}}
\newcommand{\Thetab}{\ensuremath{\bm\Theta}}
\newcommand{\Lambdab}{\ensuremath{\bm\Lambda}}
\newcommand{\Xib}{\ensuremath{\bm\Xi}}
\newcommand{\Pib}{\ensuremath{\bm\Pi}}
\newcommand{\Sigmab}{\ensuremath{\bm\Sigma}}
\newcommand{\Upsilonb}{\ensuremath{\bm\Upsilon}}
\newcommand{\Phib}{\ensuremath{\bm\Phi}}
\newcommand{\Psib}{\ensuremath{\bm\Psi}}
\newcommand{\Omegab}{\ensuremath{\bm\Omega}}
% Bold Greek Lowercase
\newcommand{\alphab}{\ensuremath{\bm\alpha}}
\newcommand{\betab}{\ensuremath{\bm\beta}}
\newcommand{\gammab}{\ensuremath{\bm\gamma}}
\newcommand{\deltab}{\ensuremath{\bm\delta}}
\newcommand{\epsilonb}{\ensuremath{\bm\epsilon}}
\newcommand{\zetab}{\ensuremath{\bm\zeta}}
\newcommand{\etab}{\ensuremath{\bm\eta}}
\newcommand{\thetab}{\ensuremath{\bm\theta}}
\newcommand{\iotab}{\ensuremath{\bm\iota}}
\newcommand{\kappab}{\ensuremath{\bm\kappa}}
\newcommand{\lambdab}{\ensuremath{\bm\lambda}}
\newcommand{\mub}{\ensuremath{\bm\mu}}
\newcommand{\nub}{\ensuremath{\bm\nu}}
\newcommand{\xib}{\ensuremath{\bm\xi}}
\newcommand{\pib}{\ensuremath{\bm\pi}}
\newcommand{\rhob}{\ensuremath{\bm\rho}}
\newcommand{\sigmab}{\ensuremath{\bm\sigma}}
\newcommand{\taub}{\ensuremath{\bm\tau}}
\newcommand{\upsilonb}{\ensuremath{\bm\upsilon}}
\newcommand{\phib}{\ensuremath{\bm\phi}}
\newcommand{\chib}{\ensuremath{\bm\chi}}
\newcommand{\psib}{\ensuremath{\bm\psi}}
\newcommand{\omegab}{\ensuremath{\bm\omega}}
\newcommand{\varepsilonb}{\ensuremath{\bm\varepsilon}}
\newcommand{\varthetab}{\ensuremath{\bm\vartheta}}
\newcommand{\varpib}{\ensuremath{\bm\varpi}}
\newcommand{\varrhob}{\ensuremath{\bm\varrho}}
\newcommand{\varsigmab}{\ensuremath{\bm\varsigma}}
\newcommand{\varphib}{\ensuremath{\bm\varphi}}
% Other Bold
\newcommand{\bma}{\ensuremath{\bm a}}
\newcommand{\bmb}{\ensuremath{\bm b}}
\newcommand{\bmc}{\ensuremath{\bm c}}
\newcommand{\bmd}{\ensuremath{\bm d}}
\newcommand{\bme}{\ensuremath{\bm e}}
\newcommand{\bmf}{\ensuremath{\bm f}}
\newcommand{\bmg}{\ensuremath{\bm g}}
\newcommand{\bmh}{\ensuremath{\bm h}}
\newcommand{\bmi}{\ensuremath{\bm i}}
\newcommand{\bmj}{\ensuremath{\bm j}}
\newcommand{\bmk}{\ensuremath{\bm k}}
\newcommand{\bml}{\ensuremath{\bm l}}
\newcommand{\bmm}{\ensuremath{\bm m}}
\newcommand{\bmn}{\ensuremath{\bm n}}
\newcommand{\bmo}{\ensuremath{\bm o}}
\newcommand{\bmp}{\ensuremath{\bm p}}
\newcommand{\bmq}{\ensuremath{\bm q}}
\newcommand{\bmr}{\ensuremath{\bm r}}
\newcommand{\bms}{\ensuremath{\bm s}}
\newcommand{\bmt}{\ensuremath{\bm t}}
\newcommand{\bmu}{\ensuremath{\bm u}}
\newcommand{\bmv}{\ensuremath{\bm v}}
\newcommand{\bmw}{\ensuremath{\bm w}}
\newcommand{\bmx}{\ensuremath{\bm x}}
\newcommand{\bmy}{\ensuremath{\bm y}}
\newcommand{\bmz}{\ensuremath{\bm z}}
\newcommand{\bmA}{\ensuremath{\bm A}}
\newcommand{\bmB}{\ensuremath{\bm B}}
\newcommand{\bmC}{\ensuremath{\bm C}}
\newcommand{\bmD}{\ensuremath{\bm D}}
\newcommand{\bmE}{\ensuremath{\bm E}}
\newcommand{\bmF}{\ensuremath{\bm F}}
\newcommand{\bmG}{\ensuremath{\bm G}}
\newcommand{\bmH}{\ensuremath{\bm H}}
\newcommand{\bmI}{\ensuremath{\bm I}}
\newcommand{\bmJ}{\ensuremath{\bm J}}
\newcommand{\bmK}{\ensuremath{\bm K}}
\newcommand{\bmL}{\ensuremath{\bm L}}
\newcommand{\bmM}{\ensuremath{\bm M}}
\newcommand{\bmN}{\ensuremath{\bm N}}
\newcommand{\bmO}{\ensuremath{\bm O}}
\newcommand{\bmP}{\ensuremath{\bm P}}
\newcommand{\bmQ}{\ensuremath{\bm Q}}
\newcommand{\bmR}{\ensuremath{\bm R}}
\newcommand{\bmS}{\ensuremath{\bm S}}
\newcommand{\bmT}{\ensuremath{\bm T}}
\newcommand{\bmU}{\ensuremath{\bm U}}
\newcommand{\bmV}{\ensuremath{\bm V}}
\newcommand{\bmW}{\ensuremath{\bm W}}
\newcommand{\bmX}{\ensuremath{\bm X}}
\newcommand{\bmY}{\ensuremath{\bm Y}}
\newcommand{\bmZ}{\ensuremath{\bm Z}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                  Probability                                 %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Basic operators and standard notation
\usepackage{amsmath}
\DeclareMathOperator{\pr}{\textsf{P}}
\DeclareMathOperator{\E}{E}
\DeclareMathOperator{\var}{var}
\DeclareMathOperator{\cov}{cov}
\DeclareMathOperator{\sd}{sd}
\DeclareMathOperator{\as}{a.s.}
\DeclareMathOperator{\iid}{\overset{iid}{\sim}}
% Stochastic convergence and stochastic orders
\newcommand{\asto}{\ensuremath{\overset{\mathrm{a.s.}}{\rightarrow}}}
\newcommand{\pto}{\ensuremath{\underset{\mathrm{p}}{\rightarrow}}}
\newcommand{\dto}{\ensuremath{\overset{\mathrm{d}}{\rightarrow}}}
\newcommand{\wto}{\ensuremath{\rightsquigarrow}}
\newcommand{\op}{\ensuremath{o_{\mathrm{p}}(1)}}
\newcommand{\Op}{\ensuremath{O_{\mathrm{p}}(1)}}
% Stochastic processes
\newcommand{\m}{\ensuremath{\overset{\mathrm{m}}{=}}} % equality of marginals
\newcommand{\dd}{\ensuremath{\overset{\mathrm{d}}{=}}} % equality of joints 
\DeclareMathOperator{\GP}{\text{GP}}
\DeclareMathOperator{\DP}{\text{DP}}
\DeclareMathOperator{\PT}{\text{PT}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                  Statistics                                  %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{mathrsfs}
\DeclareMathOperator{\CI}{CI}
\newcommand{\Lik}{\mathscr{L}}
\newcommand{\hatF}{\ensuremath{\widehat{F}}} 
% Distributions
\DeclareMathOperator{\Beta}{Beta}
\DeclareMathOperator{\Bern}{Bern}
\DeclareMathOperator{\Bin}{Bin}
\DeclareMathOperator{\Dir}{Dir}
\DeclareMathOperator{\Exp}{Exp}
\DeclareMathOperator{\Ga}{Gamma}
\DeclareMathOperator{\GEV}{GEV}
\DeclareMathOperator{\GPD}{GPD}
\DeclareMathOperator{\Poi}{Poi}
\DeclareMathOperator{\IG}{IGamma}
\DeclareMathOperator{\U}{Unif}
\DeclareMathOperator{\Unif}{Unif}
\DeclareMathOperator{\Weib}{Weibull}
% Probability mass function and densities
\newcommand{\dbeta}[3]{\ensuremath{\frac{1}{B(#2,#3)} #1^{#2 - 1} 
    (1 - #1)^{#3 - 1}}}
\newcommand{\dbern}[2]{\ensuremath{#2^{#1} (1 - #2)^{1 - #1}}}
\newcommand{\dbin}[3]{\ensuremath{\binom{#2}{#1} #3^{#1} (1 - #3)^{#2 - #1}}} 
\newcommand{\ddir}[3]{\ensuremath{\frac{1}{B(\bm{#2})}\prod_{i = 1}^{#3} 
    #1_i^{#2_i - 1}}}
\newcommand{\dexp}[2]{\ensuremath{#2 \exp\lbrace-#2 #1 \rbrace}}
\newcommand{\dexpf}[2]{\ensuremath{\frac{1}{#2} \exp\lbrace -\frac{#1}{#2} 
    \rbrace}}
\newcommand{\dgamma}[3]{\ensuremath{\frac{#3^{#2}}{\Gamma(#2)}{#1}^{#2 - 1}\exp(-#3 #2)}}
\newcommand{\dgammaf}[3]{\ensuremath{\frac{1}{\Gamma{#2}#3^{#2}} #1^{#2 - 1} 
    \exp(-#1/#2)}}
\newcommand{\dnorm}[3]{\ensuremath{\frac{1}{#3\sqrt{2\pi}} 
    \exp\Bigl\lbrace -\frac{1}{2} \Bigl(\frac{#1 - #2}{#3}\Bigr)^2 
    \Bigr\rbrace}}
% Distribution functions
\newcommand{\pexp}[2]{\ensuremath{1 - \exp\lbrace -#2 #1 \rbrace}}
\newcommand{\pgev}[4]{\ensuremath{\exp\bigl[-\Bigl\lbrace 1 + 
    #4 \bigl(\frac{#1 - #2}{#3} \bigr) \Bigr\rbrace^{-1/#4}\bigr]}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                   Computing                                  %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\R}{R}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                               Biostatistics                                  %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\DeclareMathOperator{\ROC}{ROC}
\DeclareMathOperator{\ODC}{ODC}
\DeclareMathOperator{\AUC}{AUC}
\DeclareMathOperator{\YI}{YI}

\newcommand{\D}{\ensuremath{\bar{D}}}

% % Finance
% \newcommand{\VaR}{\text{VaR}}

% Space
\newcommand{\vs}{\vspace{0.2cm}}
\newcommand{\vS}{\vspace{0.4cm}}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
\newcommand*{\Scale}[2][4]{\scalebox{#1}{$#2$}}
%%% End:

